CYGNUS: Feasibility of a nuclear recoil observatory with directional sensitivity to dark matter and neutrinos

Now that conventional weakly interacting massive particle (WIMP) dark matter searches are approaching the neutrino floor, there has been a resurgence of interest in detectors with sensitivity to nuclear recoil directions. A large-scale directional detector is attractive in that it would have sensitivity below the neutrino floor, be capable of unambiguously establishing the galactic origin of a purported dark matter signal, and could serve a dual purpose as a neutrino observatory. We present the first detailed analysis of a 1000 m$^3$-scale detector capable of measuring a directional nuclear recoil signal at low energies. We propose a modular and multi-site observatory consisting of time projection chambers (TPCs) filled with helium and SF$_6$ at atmospheric pressure. Depending on the TPC readout technology, 10-20 helium recoils above 6 keVr or only 3-4 recoils above 20 keVr would suffice to distinguish a 10 GeV WIMP signal from the solar neutrino background. High-resolution charge readout also enables powerful electron background rejection capabilities well below 10 keV. We detail background and site requirements at the 1000 m$^3$-scale, and identify materials that require improved radiopurity. The final experiment, which we name CYGNUS-1000, will be able to observe 10-40 neutrinos from the Sun, depending on the final energy threshold. With the same exposure, the sensitivity to spin independent cross sections will extend into presently unexplored sub-10 GeV parameter space. For spin dependent interactions, already a 10 m$^3$-scale experiment could compete with upcoming generation-two detectors, but CYGNUS-1000 would improve upon this considerably. Larger volumes would bring sensitivity to neutrinos from an even wider range of sources, including galactic supernovae, nuclear reactors, and geological processes.

==> design.tex <==
% !TEX root = ./paper.tex

The aim of this work has been to deliver a first thorough study of the feasibility and sensitivity of a TPC-based directional WIMP search able to reach below the neutrino floor, based on experimental detector realities (as far as known), rather than on theoretical idealized concepts as have previously been undertaken, and which are summarized in Ref.~\cite{Mayet:2016zxu}. A particular focus has been a cost/benefit analysis of different readout concepts and a realistic analysis of intrinsic backgrounds, active electron rejection and directional sensitivity. Our prime conclusion is that despite significant technical challenges Cygnus is feasible in line with the sensitivities outlined in Fig.~\ref{fig:limits}.  
Subsequent papers will begin to produce to a full conceptual design that follows the conclusions laid out in this work.
	
We envisage a TPC with total volume of 1000~m${^{3}}$, where this volume would be best achieved using multiple smaller detectors, say of $5 \times 5 \times 10$~m, located at multiple underground sites. This is sufficient in principle to meet the sensitivity goals, allows for control of systematics by comparison between experiments, and importantly, leaves room for future expansion at each site.  Utilizing multiple detectors would allow use of multiple target gases and pressures, but the currently favored scenario is to include a negative-ion drift gas, preferably SF$_{6}$.  This ensures $z$-fiducialization via minority carriers (see Sec.~\ref{sec:}) and allows for larger (>25 cm) drift distances so as to reduce readout costs.  

A further advance reached in this work is to include operation at atmospheric pressure by adding helium.  This improves the low WIMP mass and neutrino sensitivity but also avoids the need for a vacuum vessel (see Sec.~\ref{sec:sites}).   The intrinsic gamma radioactivity of the detector containment material is reduced to an acceptable <10$^{3}$ TPC detected events per year (1--10 keV).  This in turn allows us more flexibility with the gamma shielding material.  We envisage vessels with a skeletal design using low background titanium, copper and acrylic, surrounded by an inner layered structure of gamma shielding, incorporating copper and steel.  Shielding from neutron backgrounds can be achieved by using water blocks outside the inner shield (see Fig. \ref{fig:DRIFT_shield}) and a conventional muon veto depending on site depth.  Some improvement in copper radiopurity will be needed for the shielding but a back-up to this would be to use all water shielding.
	
The new simulations presented here, validated in part by experiment, suggest that electron rejection is feasible down to 1 \kevee{} in the atmospheric pressure SF$_{6}$:He mixture.  The discrimination power depends on the sophistication of the readout but is of order >10$^{5}$ at 10 \kevee.  This is achieved in the nominal SF$_{6}$:He gas mixture scenario. A pixel-chip based readout achieves the best directional sensitivity. However, the intrinsic gamma background from such a readout would require a reduction in the U/Th content of state-of-the-art devices of ~$\times{10^{5}}$.  This may be achievable in the future but alternative, simpler 2D or 1D with head-tail readouts, can already achieve sufficiently lower intrinsic backgrounds.  However, these require more sophisticated analysis techniques to reach the required active electron rejection. MIMAC \cite{Riffard:2016mgw} for instance have proposed machine learning techniques for such a task.  The optimization between intrinsic background and sophistication of readout is the subject of future work.
	
Finally, control of background events from radon and radon progeny recoils (RPRs) is a major issue in all dark matter experiments.  In Cygnus we find the main challenge to be RPRs from the central high voltage cathode.  To tackle this we envisage a combination of $z$-fiducialization and use of ultra-thin cathodes, as demonstrated in DRIFT.  We envisage further active reduction of radon by scrubbing of the gas with filters, as demonstrated in SF$_{6}$ in Ref.~\cite{Ezeribe:2017phs}.  We also envisage recirculation of the target gas through purification filters to control build up of electron-negative contaminants and to obviate any need to discharge gases to the atmosphere, thereby also saving costs.
	
	

